A Mathematical Exploration of Why Language Models Help Solve Downstream Tasks

Autoregressive language models, pretrained using large text corpora to do well on next word prediction, have been successful at solving many downstream tasks, even with zero-shot usage. However, there is little theoretical understanding of this success. This paper initiates a mathematical study of this phenomenon for the downstream task of text classification by considering the following questions: (1) What is the intuitive connection between the pretraining task of next word prediction and text classification? (2) How can we mathematically formalize this connection and quantify the benefit of language modeling? For (1), we hypothesize, and verify empirically, that classification tasks of interest can be reformulated as sentence completion tasks, thus making language modeling a meaningful pretraining task. With a mathematical formalization of this hypothesis, we make progress towards (2) and show that language models that are $\epsilon$-optimal in cross-entropy (log-perplexity) learn features that can linearly solve such classification tasks with $\mathcal{O}(\sqrt{\epsilon})$ error, thus demonstrating that doing well on language modeling can be beneficial for downstream tasks. We experimentally verify various assumptions and theoretical findings, and also use insights from the analysis to design a new objective function that performs well on some classification tasks.

==> _experiments.tex <==
% !TEX root = main.tex

\begin{figure}
\centering
	\includegraphics[scale=0.3]{img/plt_three_big.png}
	\caption{Fit of the learned quadratic function to the log partition function for features computed by GPT-2. We also plot the $y=x$ line for reference.}
	\label{fig:logZ_fit}
\end{figure}

%\subsection{Tasks solved as linear functions of $\lmp$}
\paragraph{Tasks using linear function of $\lmp$:}
\label{subsec:few_words}
We validate our claims that classification tasks can be solved by linear functions of $\lmp$ (see \Secref{sec:intuition}).
Table \ref{tab:zeroshot} on the Stanford Sentiment Treebank (SST) \citep{socher2013recursive} and AG News \citep{zhang2015character} tasks demonstrates that we can use features $\embfn$ and conditional probabilities $\lmp=p_{\embfn(s)}$ from GPT-2 \citep{radford2019language} to linearly solve tasks reasonably well.
In fact, using around 20 intuitively task-relevant tokens, or even just one token per class, yields non-trivial performance. 
%Columns 3 and 4 in Table \ref{tab:zeroshot} show that we can achieve non-trivial performance using $p_{\embfn(s)}$ over 20 or fewer task-relevant tokens, or even $p_{\embfn(s)}$ over just one token per class, selected intuitively (see \Secref{apdx:subsec:f_Phi_pf}).
%Even using the probabilities of just one word per class gives non-trivial performance.
%Furthermore, we add task-specific prompts to each input of the downstream task and extract probabilities, as discussed in \Secref{subsec:task_intuition}.
%This boosts performance, as the complete-the-sentence intuition suggests.
Furthermore, we validate the complete-the-sentence intuition in \Secref{subsec:task_intuition} by measuring probabilities after a prompt and reporting improved performance.

\input{tables/pretrained_downstream}






%\subsection{$\phip{\embfn}$ and $\embfn$ are good features}
\paragraph{$\phip{\embfn}$ and $\embfn$ are good features:}\label{subsec:newobj_exps}
We validate \Thmref{thm:robust_softmax_lm} by verifying that the conditional mean features $\phip{\embfn}(s) = \Phi p_{\embfn(s)}$ also linearly solve downstream tasks reasonably well.
This performance is comparable to, but always worse than, $\embfn(s)$, seen in columns 2 and 3 of Table \ref{tab:zeroshot}.
We again find that adding a prompt improves performance.  % of both the features.
\Secref{apdx:subsec:new_obj} has results for more classification tasks.
%
%We show guarantees for $\embfn$ in \Corref{cor:f_star_good} by using \Asmpref{asmp:partition_quadratic}.
Evidence for \Asmpref{asmp:partition_quadratic} is provided by learning a quadratic function to fit the log partition function of features from the pretrained GPT-2 model (see \Secref{apdx:subsec:f_Phi_pf}).
\Figref{fig:logZ_fit} demonstrates that the fit holds for its training and unseen data (e.g., WebText \citep{radford2019language}).
%\Secref{apdx:subsec:f_Phi_pf} has details about how the quadratic function is learned.



%\subsection{{\objname} objective}\label{subsec:quad_exps}
\paragraph{{\objname} objective:}\label{subsec:quad_exps}
We compare downstream performance of the {\objname} objective to the cross-entropy objective by training GPT-2 on the IMDb dataset \citep{maas2011learning}.
%When training with {\objname}, we use either a fixed, pre-trained $\Phi$ or learn $\Phi$. %, as presented in \Thmref{thm:new_obj_sol}.
Table \ref{tab:compare_obj} shows that {\objname} performs comparably to $\Phi p_{\embfn(s)}$ for $\embfn$ learned by the cross-entropy objective, which validates our theory that both are linear functions of $\truep$.
%both of which are linear functions of $\truep$ from our theory.
We reiterate that these experiments are intended only to demonstrate how theoretical insights can motivate the design of new objectives.
%the point of this experiment is mostly to demonstrate how insights from theory can help design new objectives.

==> _extensions.tex <==
% !TEX root = main.tex

\subsection{Better handling of distributional shift}\label{subsec:dist_shift}
The bounds above use $\gamma(\pT)$ to transfer from the distribution $\pstar$ to $\pT$ and we define a more refined notion of transferability here.
Since $\gamma(\pT)$ depends only on $\pstar$ and $\pT$, it cannot exploit any properties of the learned model to get improved guarantees, unlike the new notion.
\revise{not sure what ``new notion'' means}
% notions depend also on the learned model, thus potentially exploiting some of its inductive biases.
We first define the error made in predicted probabilities by a softmax language model $\embfn$ as $\Delta_{\{p_{\embfn(s)}\}}(s) = p_{\embfn(s)} - \truep$.
For any distribution $p\in\Delta_S$, we define the covariance\footnote{This is not exactly the covariance, but all results hold even for the standard definition of covariance.} of a function $g:\gS\rightarrow\R^D$ as $\Sigma_{p}(g) = \ex_{s\sim p} \left[g(s)g(s)^\top\right]$.
The refined transferability coefficient is defined as
\begin{align*}
    	\gamma(p; \phip{\embfn})
	&\coloneqq \left(\left\|\Sigma_{\pstar}(\Phi\Delta_{\{p_{\embfn(s)}\}})^{-\half} \Sigma_{p}(\Phi\Delta_{\{p_{\embfn(s)}\}}) \Sigma_{\pstar}(\Phi\Delta_{\{p_{\embfn(s)}\}})^{-\half}\right\|_2\right)^{-1}
\end{align*}
We now state the result for softmax language models; detailed results can be found in \Secref{asec:gamma}.
%% Theorem
\begin{theorem}[Strengthened \Thmref{thm:robust_softmax_lm}]\label{thm:robust_softmax_lm_gen}
	For a fixed $\Phi$, let $\embfn$ be features from an $\epsilon$-optimal $d$-dimensional softmax language model, i.e. $\lxent(\embfn, \Phi) - \lxent^*(\Phi) \le \epsilon$, where $\lxent^*(\Phi)$ is defined in \Eqref{eqn:l_star_xent}.
	For a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi$, we have
	\begin{align*}
		\lclf\left(\{p_{\embfn(s)}\}\right) \le \lclf(\phip{\embfn}) \le \tau + \sqrt{\frac{2B^2\epsilon}{\gamma(\pT; \phip{\embfn})}}
	\end{align*}
\end{theorem}
%\paragraph{Discussions:}
It is easy show that $\gamma(\pT; \phip{\embfn}) \ge \gamma(\pT)$, so this is indeed a stronger bound.
The coefficient $\gamma(\pT; \phip{\embfn})$ is a measure of how error by a the language model $\embfn$ on $\pstar$ can propagate to $\pT$.
This can potentially be much smaller than $\gamma(\pT)$ due to the inductive biases of $\embfn$.
For instance, if errors made by the model are random-like, i.e. $\Delta_{\{p_{\embfn(s)}\}}(s) \sim \rho$, independently of $s$, then $\Sigma_{\pstar}(\Delta_{\{\lmp\}}) \approx \Sigma_{p}(\Delta_{\{\lmp\}}) \approx \E_{\eta\sim\rho}[\eta\eta^\top]$, making $\gamma(p; \{\lmp\}) \approx 1$.
Independence prevents language modeling error from accumulating on contexts from $\pT$, bypassing the worst case transfer of $\gamma(\pT)$.






\subsection{{\objname}: A new objective function}\label{subsec:quad}
In the previous section, we argued that features from optimal language models are linear function of $\truep$ and hence useful for natural tasks.
Here we provide an alternative way to learn a linear function of $\truep$ through an objective function that replaces $\log(Z_{\embfn(s)})$ with $\frac{1}{2} \|\Phi^\top\embfn(s)\|^2$.
\begin{align}
	\lquad(\embfn, \Phi)
	&= \ex_{s\sim \pstar} \left[\ex_{w\sim\truep} [- \theta^\top \phi_w] + \frac{1}{2} \|\Phi^\top\theta\|^2\right] = -\theta^\top\Phi\truep + \frac{1}{2} \|\Phi^\top\theta\|^2\label{eqn:quad_obj}
\end{align}
For this objective, we can derive the optimal solution $\Phi^*$ that depends on a {\em substitutability matrix}.
%% Definition
\begin{definition}\label{defn:subst_matrix}
	The substitutability matrix is defined to be $\subst \coloneqq \ex_{s\sim p^*} \left[\truep~{\truep}^\top\right]\in\R^{V\times V}$.
	If $\subst = \mU\mS\mU^\top$ is the eigendecomposition, then $\mU_d\in\R^{V\times d}$ is matrix of top $d$ eigenvectors of $\subst$.
\end{definition}
This matrix captures how substitutable pairs of words are with each other.
For instance, if two words $w$ and $w'$ have exactly the same probability of occurring for every context $s\in\gS$, then occurrences of the word $w$ can replaced with the word $w'$ and still provide a meaningful completion.
Such pairs of words, which capture the idea of synonyms, were called ``free variants'' in the work on distributional semantics \citep{harris1954distributional}.
%Such pairs of words were called ``free variants" in the work on distributional semantics \cite{harris1954distributional} and captures the notion of synonyms.
We now derive expressions for optimal solutions of the {\objname} objective.
%% Theorem
\begin{theorem}\label{thm:quad_clf}
	Let $\embfnopt, \Phi^* = \argmin_{\embfn,\Phi}\lquad(f,\Phi)$.
	Then $\Phi^* = \mB\mU_d^\top\text{, for full rank }\mB\in\R^{d\times d}$.
	Also, for a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi^*$, we have $\lclf(\embfnopt) \le \tau$.
\end{theorem}
%\begin{theorem}\label{thm:new_obj_sol}
%	The optimal solution $\embfnopt, \Phi^* = \argmin_{\embfn,\Phi}\lquad(f,\Phi)$ satisfies
%	\begin{align*}
%		\Phi^* &= \mB\mU_d^\top\text{, for full rank }\mB\in\R^{d\times d}\\
%		\embfnopt(s) &= (\Phi^*{\Phi^*}^\top)^{-\nhalf}\Phi^*\truep = \mC\mU_d^\top\truep\text{, for full rank }\mC\in\R^{d\times d}
%	\end{align*}
%	If $\Phi$ is fixed, then the optimal solution is $\embfnopt(s) = (\Phi{\Phi}^\top)^{-\nhalf}\Phi\truep$.
%\end{theorem}
%\begin{corollary}
%	Let $\embfnopt, \Phi^* = \argmin_{\embfn,\Phi}\lquad(f,\Phi)$.
%	For a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi^*$, we have $\lclf(\embfnopt) \le \tau$.
%\end{corollary}
Thus we state that the optimal word embeddings $\Phi^*$ learns the top $d$ eigendirections of $\subst$ and also has the property that synonyms will have similar embeddings.
The optimal feature $\embfnopt(s)$ is essentially $\mU_d^\top\truep$, the best $d$ dimensional projection of $\truep$, thus minimizing the information loss due to projection.
We compare the performance of {\objname} to a cross-entropy language model in \Secref{subsec:quad_exps} and find {\objname} to be reasonably effective.
%We train using the {\objname} objective function and compare its performance to a language model trained in the same setting in \Secref{subsec:quad_exps} and find it to be reasonably effective.
The goal of formulating and testing {\objname} is not to obtain state-of-the-art results, but to demonstrate that insights from theory can aid the design of new and effective algorithms with provable guarantees.


==> _guarantees.tex <==
% !TEX root = main.tex

We now show guarantees for features learned by language models on natural classification tasks.
For unconstrained models, we use the learned conditional probabilities $\lmp\in\R^V$ as features on downstream tasks, while for a softmax model $\embfn$, we show guarantees for features $\Phi p_{\embfn(s)}\in\R^d$.

%%% Subsection
\subsection{Overview of results}\label{subsec:overview}
We first present simplified versions our main results that show guarantees for $\epsilon$-optimal language models on natural classification tasks, for both the unconstrained and softmax language model settings.
While \Propref{prop:unconstrained_lm} and \Propref{prop:softmax_lm} describe properties of optimal solutions for the two parameterizations, we can never hope to learn these optimal solutions with just finite samples from the language modeling distribution.
A reasonable assumption is that the learned language model is $\epsilon$-optimal in terms of the cross-entropy objective.
In the results below, we describe what $\epsilon$-optimality means in the respective settings.
We first define optimal cross entropies.
\begin{align}
	\lxent^* = \lxent(\{\truep\}),~~\lxent^*(\Phi) = \ex_{s\sim\pstar} \left[\inf_{\theta\in\R^d} \lxents(\theta, \Phi)\right]\label{eqn:l_star_xent}
\end{align}
where $\lxent^*$ is the absolute minimum achievable cross entropy, while $\lxent^*(\Phi)$ is the minimum achievable cross entropy by a $d$-dimensional softmax language model that uses $\Phi$; clearly $\lxent^* \le \lxent^*(\Phi)$.
We first present the simplified result for unconstrained language models.
%For such models, we will use the learned conditional distributions $\lmp\in\R^V$ as features for a downstream tasks and show performance guarantees for the same.
%% Restated theorem
\begin{reptheorem}{thm:robust_unconstrained_lm}[Simplified, unconstrained]
	Let $\{\lmp\}$ be a language model that is $\epsilon$-optimal, i.e. $\lxent(\{\lmp\}) - \lxent^* \le \epsilon$, for some $\epsilon>0$.
	For a classification task $\gT$ that is $(\tau, B)$-natural, we have
	\begin{align*}
		\lclf\left(\{\lmp\}\right) \le \tau + \gO(B\sqrt{\epsilon})
	\end{align*}
\end{reptheorem}
%\vspace{-0.3in}
\paragraph{Discussion:}
This bound applies to all language models, regardless of the parametrization (e.g., $n$-gram models, softmax models), and suggests that a smaller test cross-entropy (and hence test perplexity) is desirable to guarantee good downstream performance and formalizes the intuition that better language models will be more useful for downstream tasks. %, as also observed empirically in \revise{\cite{ss}}.
The term $\epsilon$ denotes the suboptimality of the learned language model and propagates gracefully as $\gO(\sqrt{\epsilon})$ to a downstream task.
Note that we can have $\epsilon=0$ only if $\lmp=\truep$ for every $s\sim\pstar$ and this recovers \Defref{def:natural_task}.
While $\tau$ can be thought of as a small constant like 0.01, the norm bound $B$ captures the difficulty (or margin) of the task $\gT$ when solved linearly using $\{\truep\}$.
Intuitively, $B$ needs to be high enough that $\vv^\top\truep = \Omega(1)$, for $\lclf(\{\truep\}, (\vv,b))$ to be made smaller than $\tau$.
Thus if the words of interest in the support of $\vv$, described in \Secref{subsec:linear_func}, have total probability mass of $\Omega(\alpha)$ in $\truep$, then $B\sim \gO(1/\alpha)$.
It is thus desirable for a task $\gT$ to depend on a larger and more frequent set of words.
A task that depends on probabilities of rare words, will have a high value of $B$.
Adding a prompt, as described in \Secref{subsec:task_intuition}, can increase the set of indicative words, thus potentially decreasing $B$.
%\paragraph{Proof sketch:}
%The first step in showing $\lclf(\{\lmp\})$ is small is to argue that for any $(s,y)\sim\pT$ and classifier $\vv\in\R^V$, $\ell(\vv^\top\lmp, y) \le \ell(\vv^\top\truep, y) + |\vv^\top(\lmp - \truep)|$ using the 1-lipschitzness of $\ell$.
%Since $\ell(\vv^\top\truep, y)$ can be made small for a natural task, we just need to upper bound $|\vv^\top(\lmp - \truep)|$ using Holder's inequality by $\|\vv\|_{\infty} \|\lmp - \truep\|_1$.
%The term $\|\lmp - \truep\|_1$ can be in turn upper bounded by $\sqrt{2\KL(\truep, \lmp)}$ using Pinsker's inequality, which equal to $\sqrt{2\left(\lxents(\lmp) - \lxents(\truep)\right)}$ and is small due to $\epsilon$-optimality of $\{\lmp\}$.

We now present the result for the $d$-dimensional softmax language models.
%% Restated theorem
\begin{reptheorem}{thm:robust_softmax_lm}[Simplified, softmax]
	Let $\embfn$ be an $\epsilon$-optimal $d$-dimensional softmax language model, i.e. $\lxent(\embfn, \Phi) - \lxent^*(\Phi) \le \epsilon$.
	For a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi$, we have
	\begin{align*}
		\lclf\left(\{p_{\embfn(s)}\}\right) \le \lclf\left(\{\Phi p_{\embfn(s)}\}\right) \le \tau + \gO(B\sqrt{\epsilon})
	\end{align*}
\end{reptheorem}
%\vspace{-0.3in}
\paragraph{Discussion:}
The conclusion is similar to that of the earlier result, that stronger language models have better downstream guarantees.
The key differences are, (1) $\epsilon$ captures the suboptimality of learned language model compared $\lxent^*(\Phi)$ and not the absolute best $\lxent^*$, (2) guarantees are for natural tasks w.r.t. $\Phi$ and not all natural tasks, due to the restriction of $d<V$.
\Thmref{thm:robust_unconstrained_lm} can also be invoked for $\{p_{\embfn(s)}\}$ to get an upper bound of $\gO(B\sqrt{\epsilon+\epsilon^*_{\Phi}})$ instead of $\gO(B\sqrt{\epsilon})$, where $\epsilon^*_{\Phi} = \lxent^*(\Phi) - \lxent^*$ is the suboptimality of the best $d$-dimensional softmax model.
Thus \Thmref{thm:robust_softmax_lm} is stronger than \Thmref{thm:robust_unconstrained_lm} for softmax language models and suggests that such language models only need to aim for optimality w.r.t. the best $d$-dimensional model.
This gain from $\gO(B\sqrt{\epsilon})$ to $\gO(B\sqrt{\epsilon+\epsilon^*_{\Phi}})$, however, comes at the cost of only having guarantees for natural tasks w.r.t. $\Phi$ as opposed to all natural tasks.
In addition to the predicted probabilities $p_{\embfn(s)}$, guarantees are also for features $\Phi p_{\embfn(s)}\in\R^d$ that we call {\em conditional mean features}.
This gives us a way to use sofmax language model features $\embfn$ to construct these $d$-dimension features that can be used for linear classification tasks, and we test the success of this mechanism experimentally in \Secref{subsec:newobj_exps}.	
%	\revise{The special case of $\epsilon=0$ gives us that $\lclf(\{\Phi p_{\embfnopt(s)}\}) \le \tau$.}
%\paragraph{Proof sketch:}
%The first step of the proof is similar: for $\lambda\in\R^d$ and $(s,y)\sim\pT$, $\ell(\lambda^\top\Phi p_{\embfn(s)}, y) \le \ell(\lambda^\top\Phi\truep, y) + |\lambda^\top(\Phi p_{\embfn(s)} - \Phi\truep)| \le \ell(\lambda^\top\Phi\truep, y) + \|\lambda\|_2 \|\Phi p_{\embfn(s)} - \Phi\truep\|_2$.
%The second term is bounded differently here, by noticing that $\nabla \lxents(\embfn(s), \Phi) = \Phi p_{\embfn(s)} - \Phi\truep$
%We then use the $\epsilon$-optimality of $\embfn$ to argue that the norm of the gradient, $\|\Phi p_{\embfn(s)} - \Phi\truep\|_2$, is small by first order optimality condition.

In the subsequent subsections we describe the results for the two settings in more detail.





%%% Subsection
\subsection{Unconstrained language models}
\label{subsec:unconstrained_lm_clf}
Language modeling guarantees that $\lmp$ is close to $\truep$ when averaged over the distribution $s\sim\pstar$.
However, the distribution $\pT$ in a classification task $\gT$ is different from $\pstar$, often a subset of it.
Thus guarantees on one distribution $\pstar$ do not directly translate to guarantees on another distribution $\pT$.
We characterize this distributional shift for downstream tasks using the following coefficient
\begin{align}
	\gamma(\pT) = \min\{\gamma\in\R : \pstar(s) \ge \gamma\pT(s)~\forall s\in\gS\}
\end{align}
This definition guarantees that $\pT$ is at least a $\gamma(\pT)$ fraction of $\pstar$, since you can write $\pstar = \gamma(\pT)\pT + (1 - \gamma(\pT))\tilde{p}_{\gT}$ for some $\tilde{p}_{\gT}\in\Delta_{\gS}$.
We now present our results.
% Theorem
\begin{theorem}\label{thm:robust_unconstrained_lm}
	Let $\{\lmp\}$ be a language model that is $\epsilon$-optimal, i.e. $\lxent(\{\lmp\}) - \lxent^* \le \epsilon$, for some $\epsilon>0$.
	For a classification task $\gT$ that is $(\tau, B)$-natural, we have
	\begin{align*}
		\lclf\left(\{\lmp\}\right) \le \tau + \sqrt{\frac{2B^2\epsilon}{\gamma(\pT)}}
	\end{align*}
\end{theorem}
\paragraph{Discussion:}
The term $\gamma(\pT)$ appears due to the shift in distribution of contexts from $\pstar$ to $\pT$.
The dependence of $1/\sqrt{\gamma(\pT)}$ is tight in some sense, when all of the $\epsilon$-error in $\lxent(\{\lmp\})$ is made on contexts from $\pT$ and no error on the rest of $\pstar$.
However this worst case dependence is unlikely to appear in practice, since the errors in practice are likely to be more evenly distributed.
Improvements over the worst case bounds are presented in \Secref{sec:dist_shit}.







%%%%% Subsection
\subsection{Softmax language model with conditional mean features}\label{subsec:eps_optimal}
We now describe guarantees for softmax language models with feature map $\embfn$.
\Propref{prop:softmax_lm} tells us that $\Phi p_{\embfnopt(s)} = \Phi \truep$ for every $s\sim\pstar$.
This mechanism of using features $\embfn(s)$ to construct $d$-dimensional features $\Phi p_{\embfn(s)}$ will be key in our analysis and we call these conditional mean features.
\begin{definition}[Conditional Mean Features]\label{def:conditional_mean_features}
	For a feature map $f:\gS\rightarrow\R^d$ and $\Phi\in\R^{d\times V}$, we define conditional mean features $\phip{\embfn}:\gS\rightarrow\R^d$, where $\phip{\embfn}(s) = \Phi p_{\embfn(s)}$, where $p_{\embfn(s)}\in\R^V$.
\end{definition}
%The above definition, in conjunction with \Propref{prop:softmax_lm}, directly gives the following results about $\phip{\embfnopt}$ for tasks that are natural w.r.t. $\Phi$.
%\begin{prop}\label{prop:f_star_good}
%	For a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi$ and satisfies $\text{supp}(\pT)\subseteq\text{supp}(\pstar)$, we have $\lclf(\phip{\embfnopt}) \le \tau$.
%\end{prop}
%This tells us that the optimal features $\embfnopt$ for a softmax language model can help solve downstream tasks through the conditional mean features $\phip{\embfnopt}$.
%We will now show an upper bound for the performance of conditional mean features $\phip{\embfn}$ from an $\epsilon$-optimal model.
\begin{theorem}\label{thm:robust_softmax_lm}
	For a fixed $\Phi$, let $\embfn$ be features from an $\epsilon$-optimal $d$-dimensional softmax language model, i.e. $\lxent(\embfn, \Phi) - \lxent^*(\Phi) \le \epsilon$, where $\lxent^*(\Phi)$ is defined in \Eqref{eqn:l_star_xent}.
	For a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi$, we have
	\begin{align*}
		\lclf\left(\{p_{\embfn(s)}\}\right) \le \lclf(\phip{\embfn}) \le \tau + \sqrt{\frac{2B^2\epsilon}{\gamma(\pT)}}
	\end{align*}
\end{theorem}
\paragraph{Discussion:}
This gives us a novel mechanism to use language model features $\embfn$ for downstream tasks, through conditional mean features $\phip{\embfn}$.
We empirically test $\phip{\embfn}$ in \Secref{subsec:newobj_exps} for features $\embfn$ from a powerful language model and find them to be effective on linear classification tasks.
This validates our theoretical findings, since apriori it is not clear why these should do well.
%\revise{fix theorem numbering in math\_commands.tex}









%%%%% Subsection
\subsection{$\phip{\embfn}(s)$ is a linear function of $\embfn(s)$}\label{subsec:linear}
%\revise{Change $\embfnopt$ to $\embfn$.}
In \Thmref{thm:robust_softmax_lm} we show that $\phip{\embfn}$ is also good for linear classification tasks.
However, the more standard way is to use the feature map $\embfn$ directly , and this has very good performance in practice as we show in \Secref{subsec:newobj_exps}.
In this section, we argue that there is a linear relation between $\embfnopt$ and $\phip{\embfnopt}$ if the word embeddings $\Phi$ satisfy certain properties.
Linearity implies that any task that can be solved linearly with $\phip{\embfn}$, can also be solved linearly using $\embfn$.
Our main assumption about the word embeddings $\Phi$ is that the logarithm of the partition function $Z_{\embfn(s)}$ is quadratic in $\embfn(s)$.
%% Assumption
\begin{assumption}\label{asmp:partition_quadratic}
	There exists a symmetric positive semidefinite matrix $\mA\in\R^{d\times d}$, a vector $\vb\in\R^d$ and a constant $c\in\R$ such that $\log(Z_{\theta}) = \half \theta^\top \mA \theta + \theta^\top \vb + c$ for any $\theta\in\R^d$.
%	\revise{This is a property of the word embeddings $\Phi$. This holds in practice ``on average", i.e. we can find a symmetric matrix $\mA$, $\vb$ and c that can fit log partition function for $\theta$s of interest (embeddings for downstream task sentences and the language model corpus contexts). This fit is quite good (refer \Figref{fig:logZ_fit}).}
\end{assumption}
%\begin{remark}
%\paragraph{Discussion:}
%\srev{Minor pt: you didn't bold matrices/vectors before}
This property is not very artificial, because when the distribution of word embedding is gaussian, i.e. $V$ columns of $\Phi$ are sampled from $\gN(\mu,\Sigma)$ independently, it is not hard to show that $\log(Z_{\theta}) \approx \half \theta^\top \Sigma \theta + \theta^\top \mu + \log(V)$. We verify this property empirically in \Secref{sec:exps} by finding the best $\mA$, $\vb$ and $c$ that approximate the log partition function as well as the related linear relation.
While not exact, the fit for log-partition is quite good as evident in \Figref{fig:logZ_fit}.
%\end{remark}
Under this assumption, we can show that a linear relation exists between $\embfn$ and $\Phi p_{\embfn}$.
%% Lemma
\begin{lemma}[Linear relation]\label{lem:theta_star}
	Under \Asmpref{asmp:partition_quadratic}, any feature map $\embfn:\gS\rightarrow\R^d$ satisfies $\phip{\embfn}(s) = \mA\embfn(s) + \vb$, for all $s\in\gS$.
%    	In fact, this statement is true for all $\theta\in\R^d$, i.e. $\Phi p_{\theta} \approx \mA\theta + \vb$.
\end{lemma}
\begin{corollary}\label{cor:f_star_good}
	Using \Lemref{lem:theta_star}, for any $\epsilon$-optimal $\embfn$, as defined in \Thmref{thm:robust_softmax_lm}, for classification tasks that are $(\tau, B)$-natural w.r.t. $\Phi$ we have $\lclf(\embfn) \le \tau + \gO(\sqrt{\epsilon})$.
\end{corollary}
However, in practice, the linearity between $\embfn$ and $\phip{\embfn}$ holds only approximately.
We use the features from the pretrained GPT-2 language model \cite{radford2018improving} to measure this linear fit and use the ratio of the residual norm to the norm of $\embfn$ to quantify the quality of the linear fit.
The quantity of interest is $r = \frac{\ex_{s\sim p} \|\phip{\embfn}(s) - \mA\embfn(s) - \vb\|^2}{\ex_{s\sim p} \|\phip{\embfn}(s) - \ex_{s\sim p}[\phip{\embfn}(s)]\|^2}$ for different distributions $p$.
%\revise{use proper r-value?}
Note that smaller $r$ means a better fit and $r=0$ means a perfect fit.
These ratios are 0.28 for SST, 0.39 for AG News, and 0.18 for IMDb contexts.
Thus we see that there exists a non-trivial linear relationship between $\embfn$ and $\Phi p_{\embfn}$, however it might not be strong enough to completely explain the success of $\embfn$.
%We computed all features using the pre-trained GPT-2 model; details in appendix.
%\revise{math for metric. closer to 0 is better.}
In fact, $\embfn$ almost always performs better than $\Phi p_{\embfn}$.
% hence it is likely that this is an incomplete explanation and that this deserves further investigation.
We leave exploring this further to future work.


==> _quad.tex <==
% !TEX root = main.tex

In the previous section, we argued that features from optimal language models are linear function of $\truep$ and hence useful for natural tasks.
Here we provide an alternative way to learn a linear function of $\truep$ through an objective function that replaces $\log(Z_{\embfn(s)})$ with $\frac{1}{2} \|\Phi^\top\embfn(s)\|^2$.
\begin{align}
	\lquads(\theta,\Phi) &= \ex_{w\sim\truep} [- \theta^\top \phi_w] + \frac{1}{2} \|\Phi^\top\theta\|^2 = -\theta^\top\Phi\truep + \frac{1}{2} \|\Phi^\top\theta\|^2\\
	\lquad(\embfn, \Phi) &= \ex_{s\sim \pstar} \left[\lquads(\embfn(s), \Phi)\right]\label{eqn:new_obj}
\end{align}
For this objective, we can derive both the optimal features $\embfnopt$ and word embeddings $\Phi^*$.
The optimal solution $\Phi^*$ depends on a {\em substitutability matrix} defined below.
%% Definition
\begin{repdefinition}{defn:subst_matrix}
	The substitutability matrix is defined to be $\subst \coloneqq \ex_{s\sim p^*} \left[\truep~{\truep}^\top\right]\in\R^{V\times V}$.
	If $\subst = \mU\mS\mU^\top$ is the eigendecomposition, then $\mU_d\in\R^{V\times d}$ is matrix of top $d$ eigenvectors of $\subst$.
\end{repdefinition}
This matrix captures how substitutable pairs of words are with each other.
For instance, if two words $w$ and $w'$ have exactly the same probability of occurring for every context $s\in\gS$, then occurrences of the word $w$ can replaced with the word $w'$ and still provide a meaningful completion.
Such pairs of words were called ``free variants" in the work on distributional semantics \cite{harris1954distributional} and can capture the notion of synonyms.
The matrix $\mU_d$ captures the $d$ most important directions of $\subst$; thus $\mU^\top\truep$ is the best $d$-dimensional projection of the probability vector $\truep$, which will show up in the optimal solution of our objective.
We now derive expressions for the optimal solution of the {\objname} objective described in \Eqref{eqn:new_obj}.
We will need the matrices $\mU_d$ and $\mS$ from \Defref{defn:subst_matrix}.
%% Theorem
\begin{theorem}\label{thm:new_obj_sol}
	The optimal solution $\embfnopt, \Phi^* = \argmin_{\embfn,\Phi}\lquad(f,\Phi)$ satisfies
	\begin{align*}
		\Phi^* &= \mB\mU_d^\top\text{, for full rank }\mB\in\R^{d\times d}\\
		\embfnopt(s) &= (\Phi^*{\Phi^*}^\top)^{-\nhalf}\Phi^*\truep = \mC\mU_d^\top\truep\text{, for full rank }\mC\in\R^{d\times d}
	\end{align*}
	If $\Phi$ is fixed, then the optimal solution is $\embfnopt(s) = (\Phi{\Phi}^\top)^{-\nhalf}\Phi\truep$.
\end{theorem}
%% Theorem
\begin{reptheorem}{thm:quad_clf}
	Let $\embfnopt, \Phi^* = \argmin_{\embfn,\Phi}\lquad(f,\Phi)$.
	Then $\Phi^* = \mB\mU_d^\top\text{, for full rank }\mB\in\R^{d\times d}$.
	Also, for a classification task $\gT$ that is $(\tau, B)$-natural w.r.t. $\Phi^*$, we have $\lclf(\embfnopt) \le \tau$.
\end{reptheorem}
Thus we get that the optimal word embeddings $\Phi^*$ learns the top $d$ eigendirections of $\subst$ and the optimal feature $\embfnopt(s)$ is a linear function of $\mU_d^\top\truep$ that is the best $d$ dimensional projection of $\truep$, thus minimizing the loss of information due to the projection.
\Thmref{thm:quad_clf} follows directly from \Thmref{thm:new_obj_sol} by observing that for any classifier $\lambda\in\R^d$ on $\Phi\truep$, we have $\lambda^\top\Phi\truep = \lambda^\top\mB^{-1}\embfnopt(s)$ and hence can be expressed as a linear function of $\embfnopt(s)$.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/phip_downstream.tex <==
% !TEX root = ../main.tex

\begin{table}[ht] % these results are in the downstream_tasks.ipynb notebook, clfs are saved by paths there
  \caption{Comparing {\objname} features to standard cross-entropy features.}
  \label{tab:compare_obj}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    Task & $\embfn(s)$ (xent) & $\Phi p_{\embfn(s)}$ (xent) & $\embfn(s)$ (\objname, fixed $\Phi$) & $\embfn(s)$ (\objname, learned $\Phi$) \\
    \midrule
    
    SST &  82.10\% & 79.90\% & 77.05\% & 77.27\% \\
    SST* & 83.08\%  & 81.05\%  & 78.47\%	 & 80.67\% \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/regression_losses.tex <==
\begin{table}[ht] % these results are in the downstream_tasks.ipynb notebook, clfs are saved by paths there
  \caption{Ratio of norm of regression error to norm of true function from fitting $\Phi p_{\embfn(s)} = A\embfn(s) + b$ using the $A$ and $b$ found through the quadratic regression shown in \Figref{fig:logZ_fit}.}
  \label{tab:reg_losses}
  \centering
  \begin{tabular}{lc}
    \toprule
    Task & Ratio of error norm to true value norm\\
    \midrule
    
    SST & 0.28 \\
    AG News & 0.39 \\
    IMDb & 0.18 \\
    \bottomrule
  \end{tabular}
\end{table}

% SST: 0.281893
% AG news: 0.39423704
% imdb: 0.18165046

